Renormalization in tensor field theory and the melonic fixed point

This thesis focuses on renormalization of tensor field theories. Its first part considers a quartic tensor model with $O(N)^3$ symmetry and long-range propagator. The existence of a non-perturbative fixed point in any $d$ at large $N$ is established. We found four lines of fixed points parametrized by the so-called tetrahedral coupling. One of them is infrared attractive, strongly interacting and gives rise to a new kind of CFT, called melonic CFTs which are then studied in more details. We first compute dimensions of bilinears and OPE coefficients at the fixed point which are consistent with a unitary CFT at large $N$. We then compute $1/N$ corrections. At next-to-leading order, the line of fixed points collapses to one fixed point. However, the corrections are complex and unitarity is broken at NLO. Finally, we show that this model respects the $F$-theorem. The next part of the thesis investigates sextic tensor field theories in rank $3$ and $5$. In rank $3$, we found two IR stable real fixed points in short range and a line of IR stable real fixed points in long range. Surprisingly, the only fixed point in rank $5$ is the Gaussian one. For the rank $3$ model, in the short-range case, we still find two IR stable fixed points at NLO. However, in the long-range case, the corrections to the fixed points are non-perturbative and hence unreliable: we found no precursor of the large $N$ fixed point. The last part of the thesis investigates the class of model exhibiting a melonic large $N$ limit. We prove that models with tensors in an irreducible representation of $O(N)$ or $Sp(N)$ in rank $5$ indeed admit a large $N$ limit. This generalization relies on recursive bounds derived from a detailed combinatorial analysis of Feynman graphs involved in the perturbative expansion of our model.

==> CTKT/CTKT_model.tex <==
In this section, we review the $O(N)^3$ model of Klebanov and Tarnopolsky \cite{Klebanov:2016xxf}. As the zero dimensional version of the model 
has been introduced by Carrozza and Tanasa \cite{Carrozza:2015adg}, we will henceforth refer to it as the CTKT model.

We consider a real tensor field of rank $3$, $\varphi_{a_1a_2 a_3}(x)$,
transforming under $O(N)^3$ with indices distinguished by the position, and we denote $\mba = (a^1,a^2,a^3)$.
The action of the model is:\footnote{From now on repeated indices are summed.
We work in $d$ space dimensions, we denote $x,y$ and so on positions, $\int_x \equiv \int d^dx$ and
$p,q$ and so on momenta and $\int_p \equiv \int \frac{d^dp}{(2\pi)^d}$. The Fourier transform is 
$  f(p) = \int_x  e^{\im p x} f(x)$ with inverse $f(x) = \int_p  e^{-\im px} f(p)$; we denote them by the same symbol, but context and argument of the function should lift any ambiguity.
The operator product in momentum space is $\int_q f(p,q) h(q,r)$, the identity operator has kernel $ (2\pi)^d \delta(p-q)$,
and translation invariant operators in the direct space are diagonal in momentum:
\begin{align}
H(x,y) & = H(x-y) = \int_p \;  e^{ - \im p (x-y) } H(p) \;, \qquad H(p) = \int_u e^{\im p u} H(y+u,y)\crcr
H(p_1,p_2) & = \int_{x,y} e^{ - \im p_1 x - \im p_2 y} \; H(x,y) = (2\pi)^d \delta(p_1+p_2) H(p_2)
 \; . 
\end{align} 
}
\be\label{eq:action} 
\begin{split}
    S[\varphi]  & =   \frac{1}{2} \int d^dx \;   \varphi_{\mba}(x) (   - \Delta)\varphi_{\mba}(x) + S^{\rm int}[\varphi]\;,\crcr
   S^{\rm int}[\varphi]  & = \frac{ m^{2}}{2} \int d^dx \;   \varphi_{\mba}(x) \delta_{\mba \mbb} \varphi_{\mbb}(x)  + 
   \frac{ \lambda }{4 N^{3/2}} \int d^d x \;   \delta^t_{\mba \mbb\mbc\mbd} \; \varphi_{\mba}(x) \varphi_{\mbb}(x)  \varphi_{\mbc}(x) \varphi_{\mbd }(x)\crcr
       & \qquad +   \int d^d x \;  \left( \frac{ \lambda_p }{4 N^{2}} \; \delta^p_{\mba\mbb; \mbc\mbd} +  \frac{ \lambda_d }{4 N^{3}}  \; \delta^d_{\mba\mbb; \mbc\mbd } \right) \; \varphi_{\mba}(x) \varphi_{\mbb}(x)  \varphi_{\mbc}(x) \varphi_{\mbd }(x) 
     \; ,     
\end{split}
\ee 
where $\Delta=  \partial_{\mu}\partial^{\mu}$,  $\delta_{\mba \mbb}  = \prod_{i=1}^3 \delta_{a^i b^i} $ and:
\begin{align}
    \delta^t_{\mba \mbb\mbc\mbd}  = \delta_{a^1 b^1}  \delta_{c^1 d^1} \delta_{a^2 c^2}  \delta_{b^2 d^2 } \delta_{a^3 d^3}   \delta_{b^3 c^3} \;  , \quad
  \delta^p_{\mba\mbb; \mbc\mbd }= \frac{1}{3} \sum_{i=1}^3  \delta_{a^ic^i} \delta_{b^id^i} \prod_{j\neq i}  \delta_{a^jb^j}  \delta_{c^jd^j} \;,
 \quad  \delta^d_{\mba\mbb; \mbc\mbd }  = \delta_{\mba \mbb}  \delta_{\mbc \mbd} \;, 
\end{align}
where $t$ stands for \emph{tetrahedron}, $d$ for \emph{double-trace} and $p$ for \emph{pillow} pattern of contraction. Because it plays a special role below, we have distinguished the coupling $\lambda$ of the tetrahedral invariant and did not assign any subscript to it.

Using the graphical representation introduced in section \ref{sec:RT}, the quartic invariants of \eqref{eq:action} are represented in Fig.~\ref{fig:interactions}.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.7\textwidth]{ColorVertex.pdf}
 \caption{Graphical representation of the quartic $O(N)^3$ invariants. From left to right: the tetrahedron, the pillow, and the double-trace (there are three pillow contractions, distinguished by the color of the vertical edge).} \label{fig:interactions}
 \end{center}
\end{figure}


To simplify the notation, we sometimes denote $A=(\mba,x)$, $\delta_{AB} = \delta_{(\mba,x) (\mbb,y)} = \delta_{\mba \mbb} \delta(x-y)$ and $\delta(x-y) = \delta_{xy}$.
We denote bilocal operators by bold face. For instance the covariance of the theory $ \mbC$ is:
\be\label{eq:cov} 
\begin{split}
 & \mbC_{AB} = \mbC_{\mba \mbb}(x,y) = \delta_{\mba \mbb}  \; \frac{1}{ (  - \Delta) } (x,y) \equiv \delta_{\mba \mbb} \;  C(x,y)  \;, \crcr
 & C(x,y) = C(x-y) = \int_p e^{ - \im p (x-y) } C(p) \;, \qquad C(p) = \frac{1}{p^{2}}  = \int_0^{\infty} d\alpha \; e^{- \alpha p^2} \;. 
\end{split}
\ee 
The last line can be combined to give the direct space representation:
%
\be
C(x-y) = \frac{1}{(4\pi)^{d/2} } \int_0^{\infty} d\alpha \;\alpha^{-d/2 } e^{- \frac{(x-y)^2}{4 \alpha}}\;.
\ee
%

At large $N$ the theory simplifies significantly: the partition function and correlations admit a $1/N$ expansion, as we will now recall. 


\subsection{Feynman graphs and large-$N$ expansion}

\paragraph{Feynman graphs}
\label{sec:model-graphs}

The free energy (and the connected $n$-point functions) of the theory can be expanded in connected Feynman graphs $\cG$. 
We will actually use two types of graphs: 4-colored graphs and ordinary Feynman graphs.

%The representation as 4-colored graphs is standard in tensor models 
%\cite{RTM,uncoloring,Carrozza:2015adg}, and it is obtained as follows. 
%Each interaction invariant is represented a 3-colored graph, as above, and we will also call it a \emph{bubble}, as in \cite{RTM,uncoloring,Carrozza:2015adg}. The propagators are represented by edges of a new color connecting the tensors (the vertices of the bubbles), which we call $0$ (black in Fig~\ref{fig:graph}). An example of the resulting 4-colored graphs is given  in Fig.~\ref{fig:graph}.
%
%\begin{figure}[ht]
%\begin{center}
%\includegraphics[width=0.7\textwidth]{ColorGraph.pdf}
% \caption{Two Feynman graphs, with external tensor contractions equivalent to the pillow (left) and double-trace (right) invariants.} \label{fig:graph}
% \end{center}
%\end{figure}

The ordinary Feynman graphs are obtained by shrinking each bubble to a point (appropriately colored in order to still distinguish the different interaction bubbles, if necessary). An example is given in Fig.~\ref{fig:melontadpoles}, where however we omit the colors of the vertices.

While the ordinary Feynman graphs are simpler, and they are sufficient for representing Feynman integrals (which we will do later), the 4-colored graphs are useful for identifying the correct powers of $N$.
In fact, in a 4-colored graph, as explained in section \ref{sec:uncolored}, each propagator identifies the indices on its two end tensors, hence the indices circulate along the cycles of colors $0i$, which we call faces. We obtain a free sum, that is a factor $N$, per face. 
We denote $n_t(\cG)$, $n_p(\cG)$ and $n_d(\cG)$ the numbers of tetrahedral, pillow, and double-trace bubbles, and $F(\cG)$ the number of faces of $\cG$. We associate a variable $x_v$ to each bubble in $\cG$. The free energy of the model is:
\begin{align}
 {\mathcal F} & =-  \ln \bigg\{  \int [d\varphi]\; e^{-S[\varphi]}\bigg\} \\
 & = \sum_{\cG} N^{F -\frac{3}{2}n_t - 2 n_p - 3n_d}  \frac{\lambda^{n_t}}{ n_t! 4^{n_t}} \frac{\lambda_p^{n_p}}{ n_p! 12^{n_p}}   \frac{\lambda_d^{n_d}}{ n_d! 4^{n_d}} (-1)^{n_t+n_p+n_d+1} A(\cG) \int_x 1  \;, \crcr
 A(\cG)& =  
 \int \prod_{ v\neq v_0 } dx_{v} \prod_{e\in \cG } C(x_e,y_e) \;,
\end{align}
where $\cG$ runs over connected vacuum 4-colored graphs with labelled tensor vertices, $v_0$ is an arbitrary root vertex, and $x_e$ and $y_e$ denote the positions of the end vertices of the edge $e$. 

\paragraph{The $1/N$ expansion.}
The model has a $1/N$ expansion\cite{Carrozza:2015adg,Klebanov:2016xxf}. The simplest way to see this is to observe that pillow and double-trace vertices can be obtained as radiative corrections from the tetrahedral vertex: the pillow is a rung (Fig~\ref{fig:graph}, left), and the double-trace 
is a ladder made out of two rungs with different color inside their loop (Fig~\ref{fig:graph}, right). Replacing the pillow and double-trace vertices in a graph by their minimal resolution in terms of tetrahedral vertices one associates to any graph $\cG$ 
a graph $\hat \cG$ having \emph{only} tetrahedral vertices but the same scaling in $N$:
\[
 F(\cG) -\frac{3}{2}n_t(\cG) - 2 n_{p}(\cG) - 3n_{d}(\cG) =  F(\hat \cG) -\frac{3}{2}n_t( \hat \cG) \;.
\]
Starting from $\hat \cG$ one can build three \emph{jackets} \cite{expansion1,Carrozza:2015adg} ${\cal J}^i$, that is ribbon graphs\footnote{The ribbon graphs are made evident in the stranded representation, where one replaces each black line and vertex by three parallel red, green, and blue lines: a jacket ${\cal J}^i$ is then obtained by simply deleting color $i$.} obtained by ignoring the faces of color $0i$.
Each jacket has a non orientable genus $k({\cal J}^i) \ge 0$ and the number of faces\footnote{It is at this point that one uses the fact that $\hat \cG$ has only tetrahedral vertices. This construction is slightly more complicated on the original graph $\cG$, as the jackets of $\cG$ are not necessarily connected \cite{Carrozza:2015adg}.}
$ {\cal F}(\cJ^i) =  n_t(\hat \cG) + 2 - k({\cal J}^i)$.
As every face belongs to two jackets, the total number of faces of $\hat \cG$ is:
\[
 {\cal F}(\hat \cG) = \frac{3}{2} n_t(\hat \cG) + 3 - \frac{1}{2} \sum_{i} k({\cal J}^i) \; .
\]
Denoting $ \omega(\cG) = \frac{1}{2} \sum_{i} k({\cal J}^i) \ge 0$ the \emph{degree} of the original graph $\cG$, the scaling with $N$ of a connected vacuum graph is:
\[
 N^{3 - \omega(\cG)} \; .
\]

By the standard arguments \cite{critical,RTM} $\cG$ has degree zero if and only if $\hat \cG$ is melonic.
That is the leading order graphs are melonic \emph{after} substituting all the pillows and double-trace vertices by their minimal realizations in terms of 
the tetrahedral vertex. In terms of the original interactions in $\cG$, one gets \emph{melon tadpole} \cite{Benedetti:2017qxl} graphs, that is 
graphs obtained by iterated insertions of melons or tadpoles into melons or tadpoles,
see Fig.~\ref{fig:melontadpoles}. Observe that all the tadpoles are based on
either pillow or double-trace vertices, while the end vertices of the melons are tetrahedral.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.3\textwidth]{MeloTadpole.pdf}
 \caption{A melon tadpole graph, where all the invariants have been shrunk to point-like vertices.} \label{fig:melontadpoles}
 \end{center}
\end{figure}


\subsection{Beta functions and fixed points}

\comment{Redo the computations or just cite KT paper ?}

The quartic interactions are marginal in $d=4$ and relevant for $d<4$: the theory at large $N$ may flow to an IR fixed point. 
Setting $d=4-\epsilon$, and rescaling the couplings as:
\begin{equation}
g=\frac{(4\pi)^2 \tilde{g}}{N^{3/2}} \; , \; g_p=\frac{(4\pi)^2\tilde{g}_p}{N^2} \; , \; g_{d}=\frac{(4\pi)^2 \tilde{g}_d}{N^3}
\end{equation}

the beta functions of this model are:

\begin{align}
\beta_t&=-\epsilon \tilde{g}-2\tilde{g}^3 \, ,\crcr
\beta_p&= -\epsilon \tilde{g}_p+6\tilde{g}^2+\frac{2}{3}\tilde{g}_p^2-2\tilde{g}^2\tilde{g}_2 \, , \crcr
\beta_d&= -\epsilon \tilde{g}_d +\frac{4}{3}\tilde{g}_p^2+4\tilde{g}_p\tilde{g}_d+2\tilde{g}_d^2-2\tilde{g}^2\left(4\tilde{g}_p+5\tilde{g}_d\right)\, .
\end{align}

Solving these beta functions, we find for the critical couplings:
\begin{equation}
\tilde{g}=\sqrt{\epsilon/2} \; , \; \tilde{g}_p=\pm 3i \sqrt{\epsilon/2} \; , \; \tilde{g}_d=\mp i(3\pm \sqrt{3})\sqrt{\epsilon/2} \; .
\end{equation}

The pillow and double-trace couplings are thus complex at the large $N$ fixed point. 


